Toward Mention Detection Robustness with Recurrent Neural Networks

One of the key challenges in natural language processing (NLP) is to yield good performance across application domains and languages. In this work, we investigate the robustness of the mention detection systems, one of the fundamental tasks in information extraction, via recurrent neural networks (RNNs). The advantage of RNNs over the traditional approaches is their capacity to capture long ranges of context and implicitly adapt the word embeddings, trained on a large corpus, into a task-specific word representation, but still preserve the original semantic generalization to be helpful across domains. Our systematic evaluation for RNN architectures demonstrates that RNNs not only outperform the best reported systems (up to 9\% relative error reduction) in the general setting but also achieve the state-of-the-art performance in the cross-domain setting for English. Regarding other languages, RNNs are significantly better than the traditional methods on the similar task of named entity recognition for Dutch (up to 22\% relative error reduction).

==> context.tex <==
% PSTricks TeX macro
% Title: C:\Users\IBM_ADMIN\Desktop\rp\dia\context.dia
% Creator: Dia v0.97.2
% CreationDate: Sun Aug 23 02:20:34 2015
% For: tnguyen
% \usepackage{pstricks}
% The following commands are not supported in PSTricks at present
% We define them conditionally, so when they are implemented,
% this pstricks file will use them.
\ifx\setlinejoinmode\undefined
  \newcommand{\setlinejoinmode}[1]{}
\fi
\ifx\setlinecaps\undefined
  \newcommand{\setlinecaps}[1]{}
\fi
% This way define your own fonts mapping (for example with ifthen)
\ifx\setfont\undefined
  \newcommand{\setfont}[2]{}
\fi
\pspicture(3.021311,-10.260266)(18.376910,-3.238678)
\psscalebox{0.221827 -0.221827}{
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\newrgbcolor{diafillcolor}{1.000000 1.000000 1.000000}%
\psset{fillcolor=diafillcolor}
\newrgbcolor{dialinecolor}{0.443137 0.972549 0.443137}%
\psset{linecolor=dialinecolor}
\pspolygon*(50.096400,16.070000)(50.096400,19.970000)(51.196400,19.970000)(51.196400,16.070000)
\psset{linewidth=0.100000cm}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\pspolygon(50.096400,16.070000)(50.096400,19.970000)(51.196400,19.970000)(51.196400,16.070000)
\setfont{Helvetica}{0.800000}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\rput(50.646400,18.215000){\psscalebox{1 -1}{}}
\newrgbcolor{dialinecolor}{0.662745 0.662745 0.662745}%
\psset{linecolor=dialinecolor}
\psellipse*(50.643064,24.468282)(1.153364,1.201682)
\psset{linewidth=0.100000cm}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\psellipse(50.643064,24.468282)(1.153364,1.201682)
\setfont{Helvetica}{0.800000}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\rput(50.643064,24.663282){\psscalebox{1 -1}{}}
\newrgbcolor{dialinecolor}{1.000000 1.000000 1.000000}%
\psset{linecolor=dialinecolor}
\pspolygon*(50.116400,28.520000)(50.116400,33.070000)(51.216400,33.070000)(51.216400,28.520000)
\psset{linewidth=0.100000cm}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\pspolygon(50.116400,28.520000)(50.116400,33.070000)(51.216400,33.070000)(51.216400,28.520000)
\setfont{Helvetica}{0.800000}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\rput(50.666400,30.990000){\psscalebox{1 -1}{}}
\psset{linewidth=0.100000cm}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\psline(50.666400,28.520000)(50.647080,26.156787)
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\pspolygon*(50.644014,25.781800)(50.898093,26.279739)(50.647080,26.156787)(50.398110,26.283827)
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\pspolygon(50.644014,25.781800)(50.898093,26.279739)(50.647080,26.156787)(50.398110,26.283827)
\psset{linewidth=0.100000cm}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\psline(50.643100,23.266600)(50.645913,20.456803)
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\pspolygon*(50.646288,20.081803)(50.895787,20.582053)(50.645913,20.456803)(50.395788,20.581553)
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\pspolygon(50.646288,20.081803)(50.895787,20.582053)(50.645913,20.456803)(50.395788,20.581553)
\newrgbcolor{dialinecolor}{0.443137 0.972549 0.443137}%
\psset{linecolor=dialinecolor}
\pspolygon*(56.123100,16.120000)(56.123100,20.020000)(57.223100,20.020000)(57.223100,16.120000)
\psset{linewidth=0.100000cm}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\pspolygon(56.123100,16.120000)(56.123100,20.020000)(57.223100,20.020000)(57.223100,16.120000)
\setfont{Helvetica}{0.800000}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\rput(56.673100,18.265000){\psscalebox{1 -1}{}}
\newrgbcolor{dialinecolor}{0.662745 0.662745 0.662745}%
\psset{linecolor=dialinecolor}
\psellipse*(56.669764,24.518282)(1.153364,1.201682)
\psset{linewidth=0.100000cm}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\psellipse(56.669764,24.518282)(1.153364,1.201682)
\setfont{Helvetica}{0.800000}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\rput(56.669764,24.713282){\psscalebox{1 -1}{}}
\newrgbcolor{dialinecolor}{1.000000 1.000000 1.000000}%
\psset{linecolor=dialinecolor}
\pspolygon*(56.143100,28.570000)(56.143100,33.120000)(57.243100,33.120000)(57.243100,28.570000)
\psset{linewidth=0.100000cm}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\pspolygon(56.143100,28.570000)(56.143100,33.120000)(57.243100,33.120000)(57.243100,28.570000)
\setfont{Helvetica}{0.800000}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\rput(56.693100,31.040000){\psscalebox{1 -1}{}}
\psset{linewidth=0.100000cm}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\psline(56.693100,28.570000)(56.673780,26.206787)
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\pspolygon*(56.670714,25.831800)(56.924793,26.329739)(56.673780,26.206787)(56.424810,26.333827)
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\pspolygon(56.670714,25.831800)(56.924793,26.329739)(56.673780,26.206787)(56.424810,26.333827)
\psset{linewidth=0.100000cm}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\psline(56.669800,23.316600)(56.672613,20.506803)
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\pspolygon*(56.672988,20.131803)(56.922487,20.632053)(56.672613,20.506803)(56.422488,20.631553)
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\pspolygon(56.672988,20.131803)(56.922487,20.632053)(56.672613,20.506803)(56.422488,20.631553)
\newrgbcolor{dialinecolor}{0.443137 0.972549 0.443137}%
\psset{linecolor=dialinecolor}
\pspolygon*(62.163100,16.120000)(62.163100,20.020000)(63.263100,20.020000)(63.263100,16.120000)
\psset{linewidth=0.100000cm}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\pspolygon(62.163100,16.120000)(62.163100,20.020000)(63.263100,20.020000)(63.263100,16.120000)
\setfont{Helvetica}{0.800000}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\rput(62.713100,18.265000){\psscalebox{1 -1}{}}
\newrgbcolor{dialinecolor}{0.662745 0.662745 0.662745}%
\psset{linecolor=dialinecolor}
\psellipse*(62.709764,24.518282)(1.153364,1.201682)
\psset{linewidth=0.100000cm}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\psellipse(62.709764,24.518282)(1.153364,1.201682)
\setfont{Helvetica}{0.800000}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\rput(62.709764,24.713282){\psscalebox{1 -1}{}}
\newrgbcolor{dialinecolor}{1.000000 1.000000 1.000000}%
\psset{linecolor=dialinecolor}
\pspolygon*(62.183100,28.570000)(62.183100,33.120000)(63.283100,33.120000)(63.283100,28.570000)
\psset{linewidth=0.100000cm}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\pspolygon(62.183100,28.570000)(62.183100,33.120000)(63.283100,33.120000)(63.283100,28.570000)
\setfont{Helvetica}{0.800000}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\rput(62.733100,31.040000){\psscalebox{1 -1}{}}
\psset{linewidth=0.100000cm}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\psline(62.733100,28.570000)(62.713780,26.206787)
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\pspolygon*(62.710714,25.831800)(62.964793,26.329739)(62.713780,26.206787)(62.464810,26.333827)
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\pspolygon(62.710714,25.831800)(62.964793,26.329739)(62.713780,26.206787)(62.464810,26.333827)
\psset{linewidth=0.100000cm}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\psline(62.709800,23.316600)(62.712613,20.506803)
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\pspolygon*(62.712988,20.131803)(62.962487,20.632053)(62.712613,20.506803)(62.462488,20.631553)
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\pspolygon(62.712988,20.131803)(62.962487,20.632053)(62.712613,20.506803)(62.462488,20.631553)
\newrgbcolor{dialinecolor}{0.443137 0.972549 0.443137}%
\psset{linecolor=dialinecolor}
\pspolygon*(75.073100,16.120000)(75.073100,20.020000)(76.173100,20.020000)(76.173100,16.120000)
\psset{linewidth=0.100000cm}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\pspolygon(75.073100,16.120000)(75.073100,20.020000)(76.173100,20.020000)(76.173100,16.120000)
\setfont{Helvetica}{0.800000}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\rput(75.623100,18.265000){\psscalebox{1 -1}{}}
\newrgbcolor{dialinecolor}{0.662745 0.662745 0.662745}%
\psset{linecolor=dialinecolor}
\psellipse*(75.619764,24.518282)(1.153364,1.201682)
\psset{linewidth=0.100000cm}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\psellipse(75.619764,24.518282)(1.153364,1.201682)
\setfont{Helvetica}{0.800000}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\rput(75.619764,24.713282){\psscalebox{1 -1}{}}
\newrgbcolor{dialinecolor}{1.000000 1.000000 1.000000}%
\psset{linecolor=dialinecolor}
\pspolygon*(75.093100,28.570000)(75.093100,33.120000)(76.193100,33.120000)(76.193100,28.570000)
\psset{linewidth=0.100000cm}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\pspolygon(75.093100,28.570000)(75.093100,33.120000)(76.193100,33.120000)(76.193100,28.570000)
\setfont{Helvetica}{0.800000}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\rput(75.643100,31.040000){\psscalebox{1 -1}{}}
\psset{linewidth=0.100000cm}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\psline(75.643100,28.570000)(75.623780,26.206787)
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\pspolygon*(75.620714,25.831800)(75.874793,26.329739)(75.623780,26.206787)(75.374810,26.333827)
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\pspolygon(75.620714,25.831800)(75.874793,26.329739)(75.623780,26.206787)(75.374810,26.333827)
\psset{linewidth=0.100000cm}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\psline(75.619800,23.316600)(75.622613,20.506803)
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\pspolygon*(75.622988,20.131803)(75.872487,20.632053)(75.622613,20.506803)(75.372488,20.631553)
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\pspolygon(75.622988,20.131803)(75.872487,20.632053)(75.622613,20.506803)(75.372488,20.631553)
\newrgbcolor{dialinecolor}{0.443137 0.972549 0.443137}%
\psset{linecolor=dialinecolor}
\pspolygon*(81.092600,16.070000)(81.092600,19.970000)(82.192600,19.970000)(82.192600,16.070000)
\psset{linewidth=0.100000cm}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\pspolygon(81.092600,16.070000)(81.092600,19.970000)(82.192600,19.970000)(82.192600,16.070000)
\setfont{Helvetica}{0.800000}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\rput(81.642600,18.215000){\psscalebox{1 -1}{}}
\newrgbcolor{dialinecolor}{0.662745 0.662745 0.662745}%
\psset{linecolor=dialinecolor}
\psellipse*(81.639964,24.468282)(1.153364,1.201682)
\psset{linewidth=0.100000cm}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\psellipse(81.639964,24.468282)(1.153364,1.201682)
\setfont{Helvetica}{0.800000}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\rput(81.639964,24.663282){\psscalebox{1 -1}{}}
\newrgbcolor{dialinecolor}{1.000000 1.000000 1.000000}%
\psset{linecolor=dialinecolor}
\pspolygon*(81.112600,28.520000)(81.112600,33.070000)(82.212600,33.070000)(82.212600,28.520000)
\psset{linewidth=0.100000cm}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\pspolygon(81.112600,28.520000)(81.112600,33.070000)(82.212600,33.070000)(82.212600,28.520000)
\setfont{Helvetica}{0.800000}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\rput(81.662600,30.990000){\psscalebox{1 -1}{}}
\psset{linewidth=0.100000cm}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\psline(81.662600,28.520000)(81.643860,26.156788)
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\pspolygon*(81.640887,25.781800)(81.894843,26.279802)(81.643860,26.156788)(81.394859,26.283767)
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\pspolygon(81.640887,25.781800)(81.894843,26.279802)(81.643860,26.156788)(81.394859,26.283767)
\psset{linewidth=0.100000cm}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\psline(81.640000,23.266600)(81.642216,20.456803)
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\pspolygon*(81.642512,20.081803)(81.892117,20.582000)(81.642216,20.456803)(81.392118,20.581606)
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\pspolygon(81.642512,20.081803)(81.892117,20.582000)(81.642216,20.456803)(81.392118,20.581606)
\psset{linewidth=0.200000cm}
\psset{linestyle=dotted,dotsep=0.200000}
\psset{linestyle=dotted,dotsep=0.200000}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\psline(68.296400,25.820000)(73.343200,25.795000)
\psset{linewidth=0.100000cm}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\psline(51.196400,19.970000)(55.472969,23.365878)
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\pspolygon*(55.766643,23.599074)(55.219614,23.483928)(55.472969,23.365878)(55.530542,23.092363)
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\pspolygon(55.766643,23.599074)(55.219614,23.483928)(55.472969,23.365878)(55.530542,23.092363)
\psset{linewidth=0.100000cm}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\psline(57.223100,20.020000)(61.510559,23.368938)
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\pspolygon*(61.806090,23.599777)(61.258156,23.489012)(61.510559,23.368938)(61.565942,23.094971)
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\pspolygon(61.806090,23.599777)(61.258156,23.489012)(61.510559,23.368938)(61.565942,23.094971)
\psset{linewidth=0.100000cm}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\psline(62.988100,20.020000)(67.759402,23.454314)
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\pspolygon*(68.063758,23.673386)(67.511903,23.584195)(67.759402,23.454314)(67.803998,23.178386)
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\pspolygon(68.063758,23.673386)(67.511903,23.584195)(67.759402,23.454314)(67.803998,23.178386)
\psset{linewidth=0.100000cm}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\psline(76.173100,20.020000)(80.439377,23.320717)
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\pspolygon*(80.735972,23.550186)(80.187532,23.441957)(80.439377,23.320717)(80.493491,23.046496)
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\pspolygon(80.735972,23.550186)(80.187532,23.441957)(80.439377,23.320717)(80.493491,23.046496)
\newrgbcolor{dialinecolor}{0.443137 0.972549 0.443137}%
\psset{linecolor=dialinecolor}
\pspolygon*(44.020000,16.120000)(44.020000,20.020000)(45.120000,20.020000)(45.120000,16.120000)
\psset{linewidth=0.100000cm}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\pspolygon(44.020000,16.120000)(44.020000,20.020000)(45.120000,20.020000)(45.120000,16.120000)
\setfont{Helvetica}{0.800000}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\rput(44.570000,18.265000){\psscalebox{1 -1}{}}
\psset{linewidth=0.100000cm}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\psline(45.120000,20.020000)(49.214718,23.683797)
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\pspolygon*(49.494181,23.933849)(48.954863,23.786754)(49.214718,23.683797)(49.288266,23.414138)
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\pspolygon(49.494181,23.933849)(48.954863,23.786754)(49.214718,23.683797)(49.288266,23.414138)
\setfont{Helvetica}{0.800000}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\rput[l](50.252900,24.665000){\psscalebox{3 -3}{$h_1$}}
\setfont{Helvetica}{0.800000}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\rput[l](56.302900,24.715000){\psscalebox{3 -3}{$h_2$}}
\setfont{Helvetica}{0.800000}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\rput[l](62.359800,24.718300){\psscalebox{3 -3}{$h_3$}}
\setfont{Helvetica}{0.800000}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\rput[l](74.919800,24.768300){\psscalebox{3 -3}{$h_{n-1}$}}
\setfont{Helvetica}{0.800000}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\rput[l](81.290000,24.668300){\psscalebox{3 -3}{$h_n$}}
\setfont{Helvetica}{0.800000}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\rput[l](50.032900,34.220000){\psscalebox{3 -3}{$x_1$}}
\setfont{Helvetica}{0.800000}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\rput[l](55.632900,34.170000){\psscalebox{3 -3}{$x_2$}}
\setfont{Helvetica}{0.800000}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\rput[l](62.132900,34.345000){\psscalebox{3 -3}{$x_3$}}
\setfont{Helvetica}{0.800000}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\rput[l](74.832900,34.295000){\psscalebox{3 -3}{$x_{n-1}$}}
\setfont{Helvetica}{0.800000}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\rput[l](80.993600,34.245000){\psscalebox{3 -3}{$x_n$}}
\setfont{Helvetica}{0.800000}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\rput[l](44.232900,15.295000){\psscalebox{3 -3}{$o_0$}}
\setfont{Helvetica}{0.800000}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\rput[l](50.232900,15.345000){\psscalebox{3 -3}{$o_1$}}
\setfont{Helvetica}{0.800000}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\rput[l](56.282900,15.345000){\psscalebox{3 -3}{$o_2$}}
\setfont{Helvetica}{0.800000}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\rput[l](62.382900,15.295000){\psscalebox{3 -3}{$o_3$}}
\setfont{Helvetica}{0.800000}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\rput[l](74.982900,15.295000){\psscalebox{3 -3}{$o_{n-1}$}}
\setfont{Helvetica}{0.800000}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\rput[l](81.143600,15.195000){\psscalebox{3 -3}{$o_n$}}
\newrgbcolor{dialinecolor}{0.662745 0.662745 0.662745}%
\psset{linecolor=dialinecolor}
\psellipse*(20.763469,36.326681)(1.153364,1.201682)
\psset{linewidth=0.100000cm}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\psellipse(20.763469,36.326681)(1.153364,1.201682)
\setfont{Helvetica}{0.800000}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\rput(20.763469,36.521681){\psscalebox{1 -1}{}}
\newrgbcolor{dialinecolor}{1.000000 1.000000 1.000000}%
\psset{linecolor=dialinecolor}
\pspolygon*(20.236805,40.378399)(20.236805,44.928399)(21.336805,44.928399)(21.336805,40.378399)
\psset{linewidth=0.100000cm}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\pspolygon(20.236805,40.378399)(20.236805,44.928399)(21.336805,44.928399)(21.336805,40.378399)
\setfont{Helvetica}{0.800000}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\rput(20.786805,42.848399){\psscalebox{1 -1}{}}
\psset{linewidth=0.100000cm}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\psline(20.786805,40.378399)(20.767455,38.015150)
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\pspolygon*(20.764384,37.640163)(21.018470,38.138099)(20.767455,38.015150)(20.518487,38.142193)
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\pspolygon(20.764384,37.640163)(21.018470,38.138099)(20.767455,38.015150)(20.518487,38.142193)
\newrgbcolor{dialinecolor}{0.662745 0.662745 0.662745}%
\psset{linecolor=dialinecolor}
\psellipse*(26.790169,36.376681)(1.153364,1.201682)
\psset{linewidth=0.100000cm}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\psellipse(26.790169,36.376681)(1.153364,1.201682)
\setfont{Helvetica}{0.800000}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\rput(26.790169,36.571681){\psscalebox{1 -1}{}}
\newrgbcolor{dialinecolor}{1.000000 1.000000 1.000000}%
\psset{linecolor=dialinecolor}
\pspolygon*(26.263505,40.428399)(26.263505,44.978399)(27.363505,44.978399)(27.363505,40.428399)
\psset{linewidth=0.100000cm}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\pspolygon(26.263505,40.428399)(26.263505,44.978399)(27.363505,44.978399)(27.363505,40.428399)
\setfont{Helvetica}{0.800000}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\rput(26.813505,42.898399){\psscalebox{1 -1}{}}
\psset{linewidth=0.100000cm}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\psline(26.813505,40.428399)(26.794155,38.065150)
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\pspolygon*(26.791084,37.690163)(27.045170,38.188099)(26.794155,38.065150)(26.545187,38.192193)
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\pspolygon(26.791084,37.690163)(27.045170,38.188099)(26.794155,38.065150)(26.545187,38.192193)
\newrgbcolor{dialinecolor}{0.662745 0.662745 0.662745}%
\psset{linecolor=dialinecolor}
\psellipse*(32.830169,36.376681)(1.153364,1.201682)
\psset{linewidth=0.100000cm}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\psellipse(32.830169,36.376681)(1.153364,1.201682)
\setfont{Helvetica}{0.800000}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\rput(32.830169,36.571681){\psscalebox{1 -1}{}}
\newrgbcolor{dialinecolor}{1.000000 1.000000 1.000000}%
\psset{linecolor=dialinecolor}
\pspolygon*(32.303505,40.428399)(32.303505,44.978399)(33.403505,44.978399)(33.403505,40.428399)
\psset{linewidth=0.100000cm}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\pspolygon(32.303505,40.428399)(32.303505,44.978399)(33.403505,44.978399)(33.403505,40.428399)
\setfont{Helvetica}{0.800000}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\rput(32.853505,42.898399){\psscalebox{1 -1}{}}
\psset{linewidth=0.100000cm}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\psline(32.853505,40.428399)(32.834155,38.065150)
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\pspolygon*(32.831084,37.690163)(33.085170,38.188099)(32.834155,38.065150)(32.585187,38.192193)
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\pspolygon(32.831084,37.690163)(33.085170,38.188099)(32.834155,38.065150)(32.585187,38.192193)
\newrgbcolor{dialinecolor}{0.662745 0.662745 0.662745}%
\psset{linecolor=dialinecolor}
\psellipse*(47.990169,36.376681)(1.153364,1.201682)
\psset{linewidth=0.100000cm}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\psellipse(47.990169,36.376681)(1.153364,1.201682)
\setfont{Helvetica}{0.800000}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\rput(47.990169,36.571681){\psscalebox{1 -1}{}}
\newrgbcolor{dialinecolor}{1.000000 1.000000 1.000000}%
\psset{linecolor=dialinecolor}
\pspolygon*(47.463505,40.428399)(47.463505,44.978399)(48.563505,44.978399)(48.563505,40.428399)
\psset{linewidth=0.100000cm}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\pspolygon(47.463505,40.428399)(47.463505,44.978399)(48.563505,44.978399)(48.563505,40.428399)
\setfont{Helvetica}{0.800000}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\rput(48.013505,42.898399){\psscalebox{1 -1}{}}
\psset{linewidth=0.100000cm}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\psline(48.013505,40.428399)(47.994155,38.065150)
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\pspolygon*(47.991084,37.690163)(48.245170,38.188099)(47.994155,38.065150)(47.745187,38.192193)
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\pspolygon(47.991084,37.690163)(48.245170,38.188099)(47.994155,38.065150)(47.745187,38.192193)
\newrgbcolor{dialinecolor}{0.662745 0.662745 0.662745}%
\psset{linecolor=dialinecolor}
\psellipse*(54.010169,36.326681)(1.153364,1.201682)
\psset{linewidth=0.100000cm}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\psellipse(54.010169,36.326681)(1.153364,1.201682)
\setfont{Helvetica}{0.800000}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\rput(54.010169,36.521681){\psscalebox{1 -1}{}}
\newrgbcolor{dialinecolor}{1.000000 1.000000 1.000000}%
\psset{linecolor=dialinecolor}
\pspolygon*(53.483505,40.378399)(53.483505,44.928399)(54.583505,44.928399)(54.583505,40.378399)
\psset{linewidth=0.100000cm}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\pspolygon(53.483505,40.378399)(53.483505,44.928399)(54.583505,44.928399)(54.583505,40.378399)
\setfont{Helvetica}{0.800000}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\rput(54.033505,42.848399){\psscalebox{1 -1}{}}
\psset{linewidth=0.100000cm}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\psline(54.033505,40.378399)(54.014155,38.015150)
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\pspolygon*(54.011084,37.640163)(54.265170,38.138099)(54.014155,38.015150)(53.765187,38.142193)
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\pspolygon(54.011084,37.640163)(54.265170,38.138099)(54.014155,38.015150)(53.765187,38.142193)
\psset{linewidth=0.100000cm}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\psline(21.916833,36.326681)(25.150046,36.370139)
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\pspolygon*(25.525012,36.375178)(25.021697,36.618436)(25.150046,36.370139)(25.028417,36.118481)
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\pspolygon(25.525012,36.375178)(25.021697,36.618436)(25.150046,36.370139)(25.028417,36.118481)
\psset{linewidth=0.100000cm}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\psline(27.943533,36.376681)(31.190002,36.376681)
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\pspolygon*(31.565002,36.376681)(31.065002,36.626681)(31.190002,36.376681)(31.065002,36.126681)
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\pspolygon(31.565002,36.376681)(31.065002,36.626681)(31.190002,36.376681)(31.065002,36.126681)
\psset{linewidth=0.100000cm}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\psline(49.143533,36.376681)(52.370046,36.333235)
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\pspolygon*(52.745012,36.328186)(52.248423,36.584896)(52.370046,36.333235)(52.241691,36.084941)
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\pspolygon(52.745012,36.328186)(52.248423,36.584896)(52.370046,36.333235)(52.241691,36.084941)
\newrgbcolor{dialinecolor}{0.662745 0.662745 0.662745}%
\psset{linecolor=dialinecolor}
\psellipse*(14.823469,36.326681)(1.153364,1.201682)
\psset{linewidth=0.100000cm}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\psellipse(14.823469,36.326681)(1.153364,1.201682)
\setfont{Helvetica}{0.800000}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\rput(14.823469,36.521681){\psscalebox{1 -1}{}}
\psset{linewidth=0.100000cm}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\psline(15.976833,36.326681)(19.123302,36.326681)
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\pspolygon*(19.498302,36.326681)(18.998302,36.576681)(19.123302,36.326681)(18.998302,36.076681)
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\pspolygon(19.498302,36.326681)(18.998302,36.576681)(19.123302,36.326681)(18.998302,36.076681)
\psset{linewidth=0.100000cm}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\psline(33.983533,36.376681)(37.333305,36.388484)
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\pspolygon*(37.708302,36.389805)(37.207425,36.638042)(37.333305,36.388484)(37.209186,36.138045)
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\pspolygon(37.708302,36.389805)(37.207425,36.638042)(37.333305,36.388484)(37.209186,36.138045)
\psset{linewidth=0.200000cm}
\psset{linestyle=dotted,dotsep=0.200000}
\psset{linestyle=dotted,dotsep=0.200000}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\psline(37.766805,37.678399)(43.330405,37.678399)
\psset{linewidth=0.100000cm}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\psline(42.866805,36.328399)(46.350038,36.370761)
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\pspolygon*(46.725010,36.375321)(46.222007,36.619223)(46.350038,36.370761)(46.228087,36.119260)
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\pspolygon(46.725010,36.375321)(46.222007,36.619223)(46.350038,36.370761)(46.228087,36.119260)
\setfont{Helvetica}{0.800000}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\rput[l](20.220105,46.103399){\psscalebox{3 -3}{$x_1$}}
\setfont{Helvetica}{0.800000}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\rput[l](26.320105,46.103399){\psscalebox{3 -3}{$x_2$}}
\setfont{Helvetica}{0.800000}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\rput[l](32.270105,46.103399){\psscalebox{3 -3}{$x_3$}}
\setfont{Helvetica}{0.800000}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\rput[l](47.220105,46.103399){\psscalebox{3 -3}{$x_{n-1}$}}
\setfont{Helvetica}{0.800000}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\rput[l](53.470105,46.103399){\psscalebox{3 -3}{$x_n$}}
\setfont{Helvetica}{0.800000}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\rput[l](15.000105,36.124999){\psscalebox{1 -1}{}}
\setfont{Helvetica}{0.800000}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\rput[l](14.473469,36.526681){\psscalebox{3 -3}{$c_0$}}
\setfont{Helvetica}{0.800000}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\rput[l](20.463469,36.526681){\psscalebox{3 -3}{$c_1$}}
\setfont{Helvetica}{0.800000}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\rput[l](26.490169,36.576681){\psscalebox{3 -3}{$c_2$}}
\setfont{Helvetica}{0.800000}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\rput[l](32.530169,36.576681){\psscalebox{3 -3}{$c_3$}}
\setfont{Helvetica}{0.800000}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\rput[l](47.340169,36.576681){\psscalebox{3 -3}{$c_{n-1}$}}
\setfont{Helvetica}{0.800000}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\rput[l](53.710169,36.526681){\psscalebox{3 -3}{$c_n$}}
\psset{linewidth=0.100000cm}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\psclip{\pswedge[linestyle=none,fillstyle=none](82.965436,21.029457){45.543206}{154.042992}{171.013365}}
\psellipse(82.965436,21.029457)(32.203910,32.203910)
\endpsclip
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\pspolygon*(51.100230,25.689174)(51.418352,26.148846)(51.153202,26.060414)(50.923366,26.219474)
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\pspolygon(51.100230,25.689174)(51.418352,26.148846)(51.153202,26.060414)(50.923366,26.219474)
\psset{linewidth=0.100000cm}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\psclip{\pswedge[linestyle=none,fillstyle=none](73.787369,34.737291){27.974558}{178.876930}{206.008489}}
\psellipse(73.787369,34.737291)(19.781000,19.781000)
\endpsclip
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\pspolygon*(56.176907,25.727736)(56.168583,26.286691)(56.004226,26.060612)(55.724749,26.056450)
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\pspolygon(56.176907,25.727736)(56.168583,26.286691)(56.004226,26.060612)(55.724749,26.056450)
\psset{linewidth=0.100000cm}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\psclip{\pswedge[linestyle=none,fillstyle=none](54.048182,26.819101){11.746437}{355.112824}{90.262219}}
\psellipse(54.048182,26.819101)(8.305985,8.305985)
\endpsclip
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\pspolygon*(62.284417,25.739140)(62.603507,26.198141)(62.338171,26.110267)(62.108671,26.269813)
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\pspolygon(62.284417,25.739140)(62.603507,26.198141)(62.338171,26.110267)(62.108671,26.269813)
\psset{linewidth=0.100000cm}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\psclip{\pswedge[linestyle=none,fillstyle=none](61.482626,23.440704){19.614299}{11.086061}{122.600136}}
\psellipse(61.482626,23.440704)(13.869404,13.869404)
\endpsclip
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\pspolygon*(75.160755,25.738895)(75.328754,26.272071)(75.101601,26.109200)(74.835013,26.193200)
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\pspolygon(75.160755,25.738895)(75.328754,26.272071)(75.101601,26.109200)(74.835013,26.193200)
\psset{linewidth=0.100000cm}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\psclip{\pswedge[linestyle=none,fillstyle=none](65.945086,25.626081){21.571819}{1.649162}{141.483959}}
\psellipse(65.945086,25.626081)(15.253579,15.253579)
\endpsclip
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\pspolygon*(81.198939,25.690294)(81.450498,26.189512)(81.200109,26.065292)(80.950501,26.191072)
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}%
\psset{linecolor=dialinecolor}
\pspolygon(81.198939,25.690294)(81.450498,26.189512)(81.200109,26.065292)(80.950501,26.191072)
}\endpspicture
